The PITA System: Tabling and Answer Subsumption for Reasoning under Uncertainty

Many real world domains require the representation of a measure of uncertainty. The most common such representation is probability, and the combination of probability with logic programs has given rise to the field of Probabilistic Logic Programming (PLP), leading to languages such as the Independent Choice Logic, Logic Programs with Annotated Disjunctions (LPADs), Problog, PRISM and others. These languages share a similar distribution semantics, and methods have been devised to translate programs between these languages. The complexity of computing the probability of queries to these general PLP programs is very high due to the need to combine the probabilities of explanations that may not be exclusive. As one alternative, the PRISM system reduces the complexity of query answering by restricting the form of programs it can evaluate. As an entirely different alternative, Possibilistic Logic Programs adopt a simpler metric of uncertainty than probability. Each of these approaches -- general PLP, restricted PLP, and Possibilistic Logic Programming -- can be useful in different domains depending on the form of uncertainty to be represented, on the form of programs needed to model problems, and on the scale of the problems to be solved. In this paper, we show how the PITA system, which originally supported the general PLP language of LPADs, can also efficiently support restricted PLP and Possibilistic Logic Programs. PITA relies on tabling with answer subsumption and consists of a transformation along with an API for library functions that interface with answer subsumption.

==> answers.tex <==

\newpage
\appendix
\section{Answer to reviewers' comments}
\subsection{Reviewer 1}
\begin{Comment}
The mode-directed tabling of B-Prolog can also be seen as a form of
answer subsumption - perhaps this point should be briefly elaborated
and/or a reference to the relevant paper be given
\end{Comment}
We agree and have added a citation to a recent B-Prolog survey
paper~\cite{Zhou11}.
\begin{Comment}
No mention of what H and B refers to. The reader has to guess that it refers to (H)ead and (B)ody, with the help
of the transformation example.
\end{Comment}
Fixed.
\begin{Comment}
The sentence: “It is not always possible to write a program so that these requirements are met” - Shouldn’t
this be, that it is possible to write a program so that these requirements are not met.
\end{Comment}
Fixed.
\begin{Comment}
 “regular” sequences is unclear and ambiguous. The word “repeated” seems more appropriate
\end{Comment}
We agree and we replaced regular with repeated.
\begin{Comment}
The equality predicate in the possibilistic logic programming example appears a bit weird to me, i.e. the first element is
always chosen, which may be right.. (will there be just the one?). It is also a bit confusing with the unused variable T.
Perhaps the predicate should be accompanied by some explanation.
\end{Comment}
We added a short explanation.
\begin{Comment}
You conclude that, “clearly, computing the possibility is much easier than computing the probability” (a rather firm
claim) ; I would assume depends on the problem etc. It more interesting with a discussion about why the different
interpretations of the program have different performance.
\end{Comment}
We have modified this statement and added a very brief note about the
comparative complexities of the approaches at the end of Section 3,
and now refer back to it in our experimental evaluation.  

However the intuition behind the statement is as follows.  Consider
the complexity of computing the fixed point of a definite program P.
If no measures of uncertainty need to be computed, computing the fixed
point is $\cO(size(P))$.  Given a finite totally ordered possibility
space of fixed size $N$, propagating the possibility measure through
conjunctions, disjunctions and negations is constant time, so that
computing the fixed point is still $\cO(size(P))$.  However for
general PLP, computing the fixed point of $P$ is NP-hard because the
disjoint sum problem has to be solved which is known to be
NP-hard \cite{DBLP:conf/iclp/KimmigCRDR08}.

%Fabrizio -- maybe you could say something about restricted PLP -- if I
%haven't already blugeoned the point to death?

\begin{Comment}
The benchmarks in Figure 4 have some peculiarities which it would be interesting to have an explanation of:
- Why is PITA(PROB) is exponential for this problem while PITA(PROB)?
- Why is the PITA(PROB) rugged and PITA(POSS) + DET perfectly smooth?
- Is the unit of Size n. edges?
\end{Comment}
PITA(PROB) is exponential because it involves the solution of the disjoint sum problem that is necessary for computing probabilities from non-exclusive explanations. PITA(POSS) does not have this requirement and its complexity for the transitive closure problem is in the same class as for DET.

The ruggedness is due to the randomness of graphs that in some cases makes the solution of the disjoint sum problem harder. 

The unit of size is edges, we have added that.
\subsection{Reviewer 2}

\begin{Comment}
The presentation of the paper could be improved by introducing an
implicit algorithm for answering a probabilistic/possibilistic
query. In fact the authors claim that the suggested approach is not
restricted to XSB system, so if the suggested approach is presented as
a query answer algorithm, the generality of the approach could be
appreciated.
\end{Comment}
%
The PITA algorithm has two main aspects: the transformation of normal
programs; and the use of tabling with answer subsumption for query
evaluation.  Intuitively and from a top-down perspective, the PITA
transformation ensures that probabilistic or possibilistic information
is properly propagated along a given derivation path, while the use of
answer subsumption combines probabilistic or possibilistic information
from two derivation paths.

Although we agree that a summary diagram for PITA might be helpful,
space limitations do not permit its inclusion.  However, we have tried
to make the above points more clearly throughout the paper than in the
first version.

As an aside, we note that discussion on implementing tabling with
answer subsumption based on the work in ~\cite{SwiW10a} has already
begun with the implementors of YAP Prolog.  Once this is implemented,
PITA will be directly portable to YAP.

\begin{Comment}
The class of possibilistic programs is really restricted (It only
considers positive programs). The implementation of a query answer
algorithm for this class of program as explained in section 7 is more
less expected and it is not a very interesting contribution.
\end{Comment}
Our intention was to show the versatility of the approach, which can be
tailored easily to different settings. We do not claim our is a state
of the art system for possibilistic logic programs, even though it
performs well in comparison with posSmodels.

Having said this, the publicly available version of \algorithmposs{}
does compute left-to-right dynamically stratified programs
(Section~\ref{tabling}) according to the semantics of~\cite{BSCV10}.
Due to space reasons, however we have not discussed this in details.
\begin{Comment}
There are not any formal results with respect to the presented mapping. The paper does not include theorems.
\end{Comment}
The theorems with respect to PITA(PROB) were introduced in
\cite{RigSwi10-ICLP10-IC}. The theorems for PITA(IND,EXC), PITA(COUNT)
and PITA(POSS) were omitted for lack of space.  

Moreover, it is
  important to remember that this paper was submitted as a System and
  Tool Paper, which according to the ICLP call for papers should place
  {\em the emphasis on the novelty, practicality, usability and
    general availability of the systems and tools described.}
\begin{Comment}
The paper lacks of a comparison of the suggested approach with other implementations for reasoning with uncertainty. For instance, in [1], it is presented an implementation for performing probabilistic reasoning. This implementation is based on YAP-Prolog system. On the other hand, in [2], a possibilistic system which is based on SMODEL system is presented.
With respect to the language, you could also consider  [2,3,4].
\end{Comment}
ProbLog was not used in the comparison because it targets the general probabilistic case as PITA. These algorithms would be surely slower with respect to those that exploit the exclusiveness and independent assumption. On the biological graphs we did not include results for ProbLog as they are already presented in \cite{RigSwi10-ICLP10-IC}.

We have added a comparison with posSmodels [2] on the biological graphs: PITA(POSS) is faster on smaller graphs and can solve larger graphs. 

We have added references to [2,3,4].

[1] ANGELIKA KIMMIG, BART DEMOEN, LUC DE RAEDT, VÍTOR SANTOS COSTA and RICARDO ROCHA, "On the implementation of the probabilistic logic programming language ProbLog", Theory and Practice of Logic Programming (2011), 11: 235-262.

[2] NICOLAS, P., GARCIA, L., STÉPHAN, I., AND LEFÈVRE, C. 2006. Possibilistic Uncertainty Handling for Answer Set Programming. Annals of Mathematics and Artificial Intelligence 47, 1-2 (June), 139–181.

[3] Chitta Baral, Michael Gelfond, J. Nelson Rushton: Probabilistic reasoning with answer sets. TPLP 9(1): 57-144 (2009)

[4] Juan Carlos Nieves, Mauricio Osorio, Ulises Cortés: Semantics for Possibilistic Disjunctive Programs. LPNMR 2007: 315-320.

\begin{Comment}
Evaluating or comparing PITA with PRISM using the program on sequences of DNA is not enough.
The program is more or less basic and  as far as I could see it does not really includes negation. The path example is also very simple to be used in the experiments.
Of course you could use these examples but please consider other more complex problems such
as perhaps a meta-interpreter. Consider examples that use stratified as well as non-stratified
negation.
\end{Comment}
The HMM program has been used as a benchmark in many papers on probabilistic logic programming
(e.g. \cite{DBLP:journals/jair/SatoK01,DBLP:conf/iclp/MantadelisJ10,DBLP:conf/ijcai/SatoKZ05}) and it is an important testbed because of its many applications. The path example is a very challenging problem since no probabilistic algorithm is known that is able to solve all of the graphs.
Adding a different example would force us to remove one of the current ones for reasons of space, while in our opinion these examples are all meaningful and worth presenting.

\subsection{Reviewer 3}
\begin{Comment}Two different styles are used for prolog (pseudo-) code, please use the style used up to page 8 also for the rest of the paper.
\end{Comment}
Fixed.
%\begin{Comment}
%I could not follow the remark in the last paragraph of the paper on the link between PITA and SCLP (as I am not familiar with the latter).
%\end{Comment}
\begin{Comment}
The paper contains lots of typo's, many of which would have been found by just running a spell-checker. 
\end{Comment}
Fixed.             


==> hmmpicture.tex <==
\iffalse
\begin{figure}
\begin{center}
\begin{tikzpicture}[
%every node/.style={ellipse,draw,font=\scriptsize,minimum height=0.5cm,minimum width=1.8cm,top color=red!60!white,bottom color = red!60!black, drop shadow
%},
x=2.5cm,y=1cm]
%[place/.style={shape=ellipse}]
%,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=6mm},
\node [font=\tiny] (xtm2) at ( -1,1) {$\ldots$};
\node 
[ellipse,draw,font=\tiny,minimum height=0.35cm,minimum width=1.5cm,top color=red!60!white,bottom color = red!60!black, drop shadow,font=\tiny]
(xtm1) at ( 0,1) {$Q(t-1)$};
\node (xt0)
[ellipse,draw,font=\tiny,minimum height=0.35cm,minimum width=1.5cm,top color=red!60!white,bottom color = red!60!black, drop shadow,font=\tiny]
 at ( 1,1) {$Q(t)$};
\node (xtp1) 
[ellipse,draw,font=\tiny,minimum height=0.35cm,minimum width=1.5cm,top color=red!60!white,bottom color = red!60!black, drop shadow,font=\tiny]
at ( 2,1) {$Q(t+1)$};
\node [font=\tiny] (xtp2) at ( 3,1) {$\ldots$};
\node 
[ellipse,draw,font=\tiny,minimum height=0.35cm,minimum width=1.5cm,top color=red!60!white,bottom color = red!60!black, drop shadow,font=\tiny]
(ytm1) at ( 0,0) {$L(t-1)$};
\node 
[ellipse,draw,font=\tiny,minimum height=0.35cm,minimum width=1.5cm,top color=red!60!white,bottom color = red!60!black, drop shadow,font=\tiny]
(yt0) at ( 1,0) {$L(t)$};
\node
[ellipse,draw,font=\tiny,minimum height=0.35cm,minimum width=1.5cm,top color=red!60!white,bottom color = red!60!black, drop shadow,font=\tiny]
 (ytp1) at ( 2,0) {$L(t+1)$};
\path[->] (xtm2) edge  (xtm1) 
(xtm1) edge  (xt0) edge (ytm1)
 (xt0) edge  (xtp1) edge (yt0)
  (xtp1) edge   (ytp1)
   (xtp1) edge  (xtp2) ;
  \end{tikzpicture}
\end{center}
\caption{Hidden Markov model.}
\label{hmm}
%\vspace{-0.8cm}
\end{figure}
\fi

